Theories of Truly Concurrent Processes

A process is able to execute a set of actions with a predefined manner, while a truly concurrent process executes this set of actions with a manner with the flavour of true concurrency. The so-called truly concurrent process algebras bridge the true concurrency (such as Petri nets, event structures, etc), and the interleaving concurrency (such as CCS, CSP, ACP, etc). In this paper, we give truly concurrent processes testing and bisimulation semantics followed by Hennessy's great work, which inherits the trinity of operational semantics, axiomatic semantics and denotational semantics.

==> Makefile <==
# source file - no spaces after the defintion
book=book
ebook=ebook
cover=images/cover

# dvi output uses .eps figure files
dvi:
	latex ${book}
	latex ${book}
	latex ${book}


# ps output uses .eps figure files
ps:     dvi
	dvips ${book}.dvi -o ${book}.ps


# pdf output uses .pdf figure files
# for make pdf, a make clean may be necessary after a make dvi
pdf:
	pdflatex ${book}
	pdflatex ${book}
	thumbpdf ${book}
	pdflatex ${book}

# .epub to be viewed with fbreader etc
epub:
	tex4ebook -c tex4ht -i -f epub -t ${ebook}
	tex4ebook -c tex4ht -i -f epub -t ${ebook}


cover:
	exit 1; # obsolete
	jpeg2ps ${cover}.jpg > ${cover}.eps
	epstopdf ${cover}.eps
	convert ${cover}.jpg -resize 50% ${cover}_small.jpg
	jpeg2ps ${cover}_small.jpg > ${cover}_small.eps
	epstopdf ${cover}_small.eps


help:
	@echo "targets:"
	@echo "- dvi"
	@echo "- ps"
	@echo "- pdf"
	@echo "- ebook"
	@echo "- words"
	@echo "- backup"
	@echo "- xdvi"
	@echo "- cover"
	@echo "- help"
	@echo "- clean"


count:  words
words:  ps
	ps2ascii ${book}.ps| wc


xdvi:
	xdvi -keep ${book} &


backup:
	zip -9ry versions/version-`date +"%Y%m%d"`.zip * -x versions/*


# target clean is not complete
clean:
	-rm -r *~  \
	tex4ht.env \
	${book}.dvi ${book}.ps ${book}.pdf ${book}.aux ${book}.log ${book}.out ${book}.toc ${book}.tpt  \
	${ebook}.epub ${ebook}*x.png ${ebook}.4ct ${ebook}.4tc ${ebook}.aux ${ebook}.css ${ebook}.dvi ${ebook}.html ${ebook}.idv ${ebook}.lg ${ebook}.log ${ebook}.ncx ${ebook}*.html ${ebook}.tmp ${ebook}.xref content.opf ${ebook}-epub*


==> section10.tex <==
\section{Truly Concurrent GSOS Languages}\label{gsos} 
\subsection{Truly Concurrent Bisimulations}\label{tcb}

Let us recall the definition of PLTS in \cref{pomlts}.

\pomsetlts*

For $n\geq 0$ and $s=U_1\cdots U_n\in\mathsf{Pom}^*$, then $p\xrightarrow{s}q$ if and only if there exist processes $p_0,\cdots,p_n$ such that $p=p_0\xrightarrow{U_1}p_1\xrightarrow{U_2}\cdots\xrightarrow{U_{n-1}}p_{n-1}\xrightarrow{U_n}p_n=q$. For $p\in\mathsf{Proc}$ and $U\in\mathsf{Pom}$, we define:

$$\mathsf{initials}(p)\triangleq\{U\in\mathsf{Pom}|\exists q:p\xrightarrow{U}q\}$$
$$\mathsf{sort}(p)\triangleq\{U\in\mathsf{Pom}|\exists s\in\mathsf{Pom}^*,p',p''\in\mathsf{Proc}:p\xrightarrow{s}p'\xrightarrow{U}p''\}$$
$$\mathsf{derivatives}(p,U)\triangleq\{q|p\xrightarrow{U}q\}$$

A PLTS is sort-finite if and only if $\mathsf{sort}(p)$ is finite for every $p\in\mathsf{Proc}$.

\begin{definition}[Pomset synchronization tree]
The set of countably branching pomset synchronization trees over $\mathsf{Pom}$, denoted $\mathsf{ST}_{\infty}(\mathsf{Pom})$, is the set of infinitary terms generated by the following inductive definition:

$$\frac{\{U_i\in\mathsf{Pom},t_i\in\mathsf{ST}_{\infty}(\mathsf{Pom})\}_{i\in I}}{\sum_{i\in I}U_i:t_i[+\Omega]\in\mathsf{ST}_{\infty}(\mathsf{Pom})}$$

where $I$ is a countable index set, $0=\sum_{i\in\emptyset}U_i:t_i$ which stands for the one-node synchronization tree, a representation of an inactive process, $\Omega=\sum_{i\in\emptyset}U_i:t_i+\Omega$ which stands that the behaviours of the synchronization tree are completely unspecified, $[+\Omega]$ means optional inclusion of $\Omega$ as a summand.
\end{definition} 

Let $\mathsf{ST}(\mathsf{Pom})$ denote the finite synchronization tree, i.e., the above set of terms is built using only finite summations. The set of synchronization trees $\mathsf{ST}_{\infty}(\mathsf{Pom})$ can be turned into a PLTS with divergence by stipulating that, for $t\in\mathsf{ST}_{\infty}(\mathsf{Pom})$:

\begin{itemize}
  \item $t\uparrow$ if and only if $\Omega$ is a summand of $t$.
  \item $t\xrightarrow{U_i}t_i$ if and only if $U_i:t_i$ is a summand of $t$.
\end{itemize} 

In the following, we give the definitions of truly concurrent bisimulations.

\begin{definition}[Configuration]
Let $\mathcal{P}=\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS. A (finite) configuration in $\mathcal{P}$ is a (finite) consistent subset of actions $C\subseteq \mathcal{P}$, closed with respect to $\xrightarrow{U}$ (i.e. $\lceil C\rceil=C$). The set of finite configurations of $\mathcal{P}$ is denoted by $\mathcal{C}(\mathcal{P})$. For $p\in\mathsf{Proc}$, the corresponding configuration is denoted $C(p)$.
\end{definition}

\begin{definition}[Pomset, step bisimulation]\label{PSB}
Let $\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS and $p,q\in\mathsf{Proc}$. A pomset bisimulation is a relation $R\subseteq\mathsf{Proc}\times\mathsf{Proc}$, such that:

\begin{enumerate}
  \item If $(p,q)\in R$, and $C(p)\xrightarrow{U}C(p')$ then $C(q)\xrightarrow{U}C(q')$, with $U\in \mathsf{Pom}$, and $(p',q')\in R$.
  \item If $(p,q)\in R$, and $C(q)\xrightarrow{U}C(q')$ then $C(p)\xrightarrow{U}C(p')$, with $U\in \mathsf{Pom}$, and $(p',q')\in R$.
\end{enumerate}

We say that $p$, $q$ are pomset bisimilar, written $p\sim_P q$, if there exists a pomset bisimulation $R$, such that $(p,q)\in R$. By replacing pomset transitions with steps, we can get the definition of step bisimulation. When $p$ and $q$ are step bisimilar, we write $p\sim_S q$.
\end{definition}

\begin{definition}[Posetal product]
Let $\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS. Given two processes $p,q\in\mathsf{Proc}$, the posetal product of their configurations, denoted $\mathcal{C}(\mathcal{P})\overline{\times}\mathcal{C}(\mathcal{P})$, is defined as

$$\{(C(p),f,C(q))|C(p)\in\mathcal{C}(\mathcal{P}),C(q)\in\mathcal{C}(\mathcal{P}),f:C(p)\rightarrow C(q) \mbox{ isomorphism}\}$$

A subset $R\subseteq\mathcal{C}(\mathcal{P})\overline{\times}\mathcal{C}(\mathcal{P})$ is called a posetal relation. We say that $R$ is downward closed when for any $(C(p),f,C(q)),(C(p'),f',C(q'))\in \mathcal{C}(\mathcal{P})\overline{\times}\mathcal{C}(\mathcal{P})$, if $(C(p),f,C(q))\subseteq (C(p'),f',C(q'))$ pointwise and $(C(p'),f',C(q'))\in R$, then $(C(p),f,C(q))\in R$.

For $f:U\rightarrow U$, we define $f[a\mapsto a]:U\cup\{a\}\rightarrow U\cup\{a\}$, $z\in U\cup\{a\}$,(1)$f[a\mapsto a](z)=a$,if $z=a$;(2)$f[a\mapsto a](z)=f(z)$, otherwise. Where $U\in \mathsf{Pom}$, $a\in \mathsf{Act}$.
\end{definition}

\begin{definition}[(Hereditary) history-preserving bisimulation]\label{HHPB}
Let $\mathcal{P}=\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS and $p,q\in\mathsf{Proc}$. A history-preserving (hp-) bisimulation is a posetal relation $R\subseteq\mathcal{C}(\mathcal{P})\overline{\times}\mathcal{C}(\mathcal{P})$ such that:

\begin{enumerate}
  \item If $(C(p),f,C(q))\in R$, and $C(p)\xrightarrow{a} C(p')$, then $C(q)\xrightarrow{a} C(q')$, with $(C(p'),f[a\mapsto a],C(q'))\in R$.
  \item If $(C(p),f,C(q))\in R$, and $C(q)\xrightarrow{a} C(q')$, then $C(p)\xrightarrow{a} C(p')$, with $(C(p'),f[a\mapsto a],C(q'))\in R$.
\end{enumerate}

$p,q$ are history-preserving (hp-)bisimilar and are written $p\sim_{HP}q$ if there exists an hp-bisimulation $R$ such that $(\emptyset,\emptyset,\emptyset)\in R$.

A hereditary history-preserving (hhp-)bisimulation is a downward closed hp-bisimulation. $p,q$ are hereditary history-preserving (hhp-)bisimilar and are written $p\sim_{HHP}q$.
\end{definition}

In the following, we give the definitions of truly concurrent prebisimulations.

\begin{definition}[Pomset, step prebisimulation]\label{PSPB}
Let $\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS with divergence $\uparrow$ and $p,q\in\mathsf{Proc}$. Let $\mathsf{Rel}(\mathsf{Proc})$ denote the set of binary relations over $\mathsf{Proc}$. Define the functional $F:\mathsf{Rel}(\mathsf{Proc})\rightarrow\mathsf{Rel}(\mathsf{Proc})$, such that:

\begin{align*}
\begin{aligned}
F(R)=&\{(p,q)|\forall U\in\mathsf{Pom}\\
  &\bullet C(p)\xrightarrow{U}C(p')\mbox{ implies } C(q)\xrightarrow{U}C(q'), \mbox{ and }(p',q')\in R\\
  &\bullet p\downarrow\mbox{ implies }\bigg(q\downarrow\mbox{ and }\Big(C(q)\xrightarrow{U}C(q')\mbox{ implies } C(p)\xrightarrow{U}C(p'),\mbox{ and }(p',q')\in R\Big)\bigg)\}\\
\end{aligned}
\end{align*}

A relation $R$ is a pomset prebisimulation if and only if $R\subseteq F(R)$. We say that $p$, $q$ are pomset prebisimilar, written $p\prepomset q$, if there exists a pomset prebisimulation $R$, such that $(p,q)\in R$. By replacing pomset transitions with steps, we can get the definition of step prebisimulation. When $p$ and $q$ are step prebisimilar, we write $p\prestep q$.

The kernels of $\prepomset$ and $\prestep$ are denoted $\prepomseteq$ and $\prestepeq$.
\end{definition}

\begin{definition}[(Hereditary) history-preserving prebisimulation]\label{HHPPB}
Let $\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS with divergence $\uparrow$ and $p,q\in\mathsf{Proc}$. Let $\mathsf{Rel}(\mathcal{C}(\mathcal{P})\overline{\times}\mathcal{C}(\mathcal{P}))$ denote the set of posetal relations over $\mathsf{Proc}$. Define the functional $F:\mathsf{Rel}(\mathcal{C}(\mathcal{P})\overline{\times}\mathcal{C}(\mathcal{P}))\rightarrow\mathsf{Rel}(\mathcal{C}(\mathcal{P})\overline{\times}\mathcal{C}(\mathcal{P}))$, such that:

\begin{align*}
\begin{aligned}
F(R)=&\{(C(p),f,C(q))|\forall a\in\mathsf{Act}\\
  &\bullet C(p)\xrightarrow{a}C(p')\mbox{ implies } C(q)\xrightarrow{a}C(q'), \mbox{ and }(C(p'),f[a\mapsto a],C(q'))\in R\\
  &\bullet p\downarrow\mbox{ implies }\\
  &\bigg(q\downarrow\mbox{ and }\Big(C(q)\xrightarrow{a}C(q')\mbox{ implies } C(p)\xrightarrow{a}C(p'),\mbox{ and }(C(p'),f[a\mapsto a],C(q'))\in R\Big)\bigg)\}\\
\end{aligned}
\end{align*}

A relation $R$ is an hp-prebisimulation if and only if $R\subseteq F(R)$. We say that $p$, $q$ are hp-prebisimilar, written $p\prehp q$, if there exists an hp-prebisimulation $R$, such that $(\emptyset,\emptyset,\emptyset)\in R$. A hereditary history-preserving (hhp-)prebisimulation is a downward closed hp-prebisimulation. $p,q$ are hereditary history-preserving (hhp-)prebisimilar and are written $p\prehhp q$.

The kernels of $\prehp$ and $\prehhp$ are denoted $\prehpeq$ and $\prehhpeq$.
\end{definition}

By use of the functional $F$ in \cref{PSPB} and \cref{HHPPB}, we can obtain a pomset behavioural preorder which applies itself inductively as follows:

$$\prepomsets{0}\triangleq\mathsf{Proc}\times\mathsf{Proc}$$
$$\prepomsets{n+1}\triangleq F(\prepomsets{n})$$
$$\prepomsets{\omega}\triangleq\bigcap_{n\geq 0}\prepomsets{n}$$

Similarly, we can get the definitions of $\presteps{\omega}$, $\prehps{\omega}$ and $\prehhps{\omega}$.

\begin{definition}[Finitary pomset prebisimulation]
Let $\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS and $p,q\in\mathsf{Proc}$. The finitary pomset prebisimulation $\prepomset^F$ over $\mathsf{Proc}$ is defined as follows: $p\prepomset^F q$ if and only if, for every $t\in\mathsf{ST}(\mathsf{Pom})$, $t\prepomset p$ implies $t\prepomset q$.
\end{definition} 

\begin{definition}[Finitary step prebisimulation]
Let $\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS and $p,q\in\mathsf{Proc}$. The finitary step prebisimulation $\prestep^F$ over $\mathsf{Proc}$ is defined as follows: $p\prestep^F q$ if and only if, for every $t\in\mathsf{ST}(\mathsf{Pom})$, $t\prestep p$ implies $t\prestep q$.
\end{definition}

\begin{definition}[Finitary hp-prebisimulation]
Let $\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS and $p,q\in\mathsf{Proc}$. The finitary hp-prebisimulation $\prehp^F$ over $\mathsf{Proc}$ is defined as follows: $p\prehp^F q$ if and only if, for every $t\in\mathsf{ST}(\mathsf{Pom})$, $t\prehp p$ implies $t\prehp q$.
\end{definition}

\begin{definition}[Finitary hhp-prebisimulation]
Let $\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS and $p,q\in\mathsf{Proc}$. The finitary hhp-prebisimulation $\prehhp^F$ over $\mathsf{Proc}$ is defined as follows: $p\prehhp^F q$ if and only if, for every $t\in\mathsf{ST}(\mathsf{Pom})$, $t\prehhp p$ implies $t\prehhp q$.
\end{definition} 

They are obvious that $\prepomset~\subseteq~\prepomsets{\omega}~\subseteq~\prepomset^F$, $\prestep~\subseteq~\presteps{\omega}~\subseteq~\prestep^F$, $\prehp~\subseteq~\prehps{\omega}~\subseteq~\prehp^F$ and $\prehhp~\subseteq~\prehhps{\omega}~\subseteq~\prehhp^F$. Moreover, the inclusions are strict for infinitely branching PLTSs, and collapse to equalities for finitely branching PLTSs. 

Let $\langle\mathsf{Proc},\mathsf{Act},\{\xrightarrow{U}|U\in\mathsf{Pom}\},\mathsf{Pred}\rangle$ be a PLTS and $p,q\in\mathsf{Proc}$. For every $P\subseteq\mathsf{Pom}$, we define the following relations.

$\{\pretesting^{P}_{(P,n)}|n\geq 0\}$

$p\pretesting^{P}_{(P,0)}q\mbox{ if and only if } \mathrm{true}$
\begin{align*}
\begin{aligned}
&p\pretesting^{P}_{(P,n+1)}q\mbox{ if and only if }\\
  &\bullet \forall U\in P,C(p)\xrightarrow{U}C(p')\mbox{ implies } C(q)\xrightarrow{U}C(q'), \mbox{ and }p'\pretesting^{P}_{(P,n)}q'\\
  &\bullet \mathsf{initials(p)}\subseteq P\mbox{ and }p\downarrow\mbox{ imply }\\
  &\bigg(\mathsf{initials(q)}\subseteq P\mbox,q\downarrow,\Big(\forall U\in P, C(q)\xrightarrow{U}C(q')\mbox{ implies } C(p)\xrightarrow{U}C(p'),\mbox{ and }p'\pretesting^{P}_{(P,n)}q'\Big)\bigg)\\
\end{aligned}
\end{align*}

Similarly, we can get the definition of $\{\pretesting^{P}_{(S,n)}|n\geq 0\}$, $\{\pretesting^{P}_{(HP,n)}|n\geq 0\}$ and $\{\pretesting^{P}_{(HHP,n)}|n\geq 0\}$.

\begin{proposition}
For every $n\geq 0$ and $P\subseteq\mathsf{Pom}$, the following statements hold:

\begin{enumerate}
  \item $\pretesting^{P}_{(P,n)}$, $\pretesting^{P}_{(S,n)}$, $\pretesting^{P}_{(HP,n)}$ and $\pretesting^{P}_{(HHP,n)}$ are all preorders.
  \item For $p,q\in\mathsf{Proc}$, 
  \begin{enumerate}
    \item $p\pretesting^{P}_{(P,n+1)}q\mbox{ implies } p\pretesting^{P}_{(P,n)}q$.
    \item $p\pretesting^{P}_{(S,n+1)}q\mbox{ implies } p\pretesting^{P}_{(S,n)}q$.
    \item $p\pretesting^{P}_{(HP,n+1)}q\mbox{ implies } p\pretesting^{P}_{(HP,n)}q$.
    \item $p\pretesting^{P}_{(HHP,n+1)}q\mbox{ implies } p\pretesting^{P}_{(HHP,n)}q$.
  \end{enumerate}
  \item Assume that $P\subseteq P'\subseteq\mathsf{Pom}$, then for $p,q\in\mathsf{Proc}$,
  \begin{enumerate}
    \item $p\pretesting^{P'}_{(P,n)}q\mbox{ implies } p\pretesting^{P}_{(P,n)}q$.
    \item $p\pretesting^{P'}_{(S,n)}q\mbox{ implies } p\pretesting^{P}_{(S,n)}q$.
    \item $p\pretesting^{P'}_{(HP,n)}q\mbox{ implies } p\pretesting^{P}_{(HP,n)}q$.
    \item $p\pretesting^{P'}_{(HHP,n)}q\mbox{ implies } p\pretesting^{P}_{(HHP,n)}q$.
  \end{enumerate}
\end{enumerate}
\end{proposition}

We define:

$$\pretesting^{P}_{(P,\omega)}\triangleq\bigcap_{n\geq 0}\pretesting^{P}_{(P,n)}$$
$$\pretesting^{P}_{(S,\omega)}\triangleq\bigcap_{n\geq 0}\pretesting^{P}_{(S,n)}$$
$$\pretesting^{P}_{(HP,\omega)}\triangleq\bigcap_{n\geq 0}\pretesting^{P}_{(HP,n)}$$
$$\pretesting^{P}_{(HHP,\omega)}\triangleq\bigcap_{n\geq 0}\pretesting^{P}_{(HHP,n)}$$
$$p\pretesting^{fin}_{(P,\omega)}q\triangleq\forall P\subseteq_{fin}\mathsf{Pom}.p\pretesting^{P}_{(P,\omega)}q$$
$$p\pretesting^{fin}_{(S,\omega)}q\triangleq\forall P\subseteq_{fin}\mathsf{Pom}.p\pretesting^{P}_{(S,\omega)}q$$
$$p\pretesting^{fin}_{(HP,\omega)}q\triangleq\forall P\subseteq_{fin}\mathsf{Pom}.p\pretesting^{P}_{(HP,\omega)}q$$
$$p\pretesting^{fin}_{(HHP,\omega)}q\triangleq\forall P\subseteq_{fin}\mathsf{Pom}.p\pretesting^{P}_{(HHP,\omega)}q$$

where $P\subseteq_{fin}\mathsf{Pom}$ means that $P$ is a finite subset of $\mathsf{Pom}$.

\begin{lemma}
For every $t\in\mathsf{ST}(\mathsf{Pom})$ and $p\in\mathsf{Proc}$, the following statements hold:

\begin{enumerate}
  \item $t\prepomset p\mbox{ if and only if } t\pretesting^{fin}_{(P,\omega)}p$.
  \item $t\prestep p\mbox{ if and only if } t\pretesting^{fin}_{(S,\omega)}p$.
  \item $t\prehp p\mbox{ if and only if } t\pretesting^{fin}_{(HP,\omega)}p$.
  \item $t\prehhp p\mbox{ if and only if } t\pretesting^{fin}_{(HHP,\omega)}p$.
\end{enumerate}
\end{lemma}

\begin{lemma}
The following statements hold:

\begin{enumerate}
  \item The preorder $\pretesting^{fin}_{(P,\omega)}$ is finitary.
  \item The preorder $\pretesting^{fin}_{(S,\omega)}$ is finitary.
  \item The preorder $\pretesting^{fin}_{(HP,\omega)}$ is finitary.
  \item The preorder $\pretesting^{fin}_{(HHP,\omega)}$ is finitary.
\end{enumerate}
\end{lemma}

\begin{theorem}
For $p,q\in\mathsf{Proc}$ in any transition system, the following statements hold:

\begin{enumerate}
  \item $p\prepomset^{F} q\mbox{ if and only if } p\pretesting^{fin}_{(P,\omega)}q$.
  \item $p\prestep^{F} q\mbox{ if and only if } p\pretesting^{fin}_{(S,\omega)}q$.
  \item $p\prehp^{F} q\mbox{ if and only if } p\pretesting^{fin}_{(HP,\omega)}q$.
  \item $p\prehhp^{F} q\mbox{ if and only if } p\pretesting^{fin}_{(HHP,\omega)}q$.
\end{enumerate}
\end{theorem}

\begin{corollary}
For $p,q\in\mathsf{Proc}$ in any sort-finite transition system, the following statements hold:

\begin{enumerate}
  \item $p\prepomset^{F} q\mbox{ if and only if } p\prepomsets{\omega}q$.
  \item $p\prestep^{F} q\mbox{ if and only if } p\presteps{\omega}q$.
  \item $p\prehp^{F} q\mbox{ if and only if } p\prehps{\omega}q$.
  \item $p\prehhp^{F} q\mbox{ if and only if } p\prehhps{\omega}q$.
\end{enumerate}
\end{corollary} 
